Learning the Platform, Not the Learner: Sequencing Shortcuts in the Offline Evaluation of Educational Recommender Systems and LLM Rankers

Educational recommenders are usually compared offline, by how well they predict the next activity in logs of tutoring systems, learning applications and MOOCs, where the next activity is largely decided by the platform: teachers assign problem sets, tutors draw problems until mastery, engines select questions. On eight public datasets from five platforms, we compare four structural predictors, which use nothing about the learner beyond the last activity, with ten personalised recommenders and with open-weight LLM rankers from 0.5 to 7 billion parameters, under two protocols. The structural predictors reach between 0.81 and 1.00 of the best accuracy of any method (median 0.95), mostly through population transitions rather than the course order; the best personalised recommender is significantly better on five datasets, by 0.007 to 0.102 NDCG@10, and on Eedi in three of four training runs. Every method is far less accurate on steps along transitions never seen in training and on steps chosen by learners. LLM rankers look competent with random negatives but are never much better than a word-matching baseline, and with negatives that are plausible under the course structure they stay close to random or well behind the transition heuristic, whatever their size. In a simulation with known learner needs, the structural share tracks the share of steps decided by the platform, and offline accuracy ranks an oracle of the learners' needs below imitators of the platform. Weighting test steps by how unlikely the structure makes them restores much of the link with usefulness and, on the real data, reveals a significant personalisation signal on seven of the eight datasets. We propose a syllabus-aware evaluation checklist and release a Python package that reports the lift of any recommender over the structure.

==> tables/main_hr10_lift.tex <==
\begin{tabular}{llrlrrrrr}
\toprule
Dataset & Best structural & $S_{\text{struct}}$ & Best personalised & Score & $\Delta$ [95\% interval] & $p_{\text{Holm}}$ & $\rho$ & $\rho_{\text{meta}}$ \\
\midrule
A09 & CONT & 0.173 & ItemKNN & 0.146 & -0.027 [-0.040, -0.013] & $<$0.001 & 1.00 & 1.00 \\
A12 & MC & 0.346 & SASRec & 0.315 & -0.031 [-0.036, -0.027] & $<$0.001 & 1.00 & 0.36 \\
A15 & MC & 0.631 & SASRec & 0.730 & +0.100 [+0.093, +0.107] & $<$0.001 & 0.86 & 0.29 \\
A17 & MC & 0.779 & SASRec & 0.786 & +0.007 [-0.003, +0.017] & 0.354 & 0.99 & 0.43 \\
EdNet & MC & 0.067 & SASRec & 0.083 & +0.016 [+0.008, +0.025] & $<$0.001 & 0.80 & 0.26 \\
Junyi & MC & 0.631 & SASRec & 0.671 & +0.040 [+0.035, +0.045] & $<$0.001 & 0.94 & 0.65 \\
Eedi & MC & 0.824 & SASRec & 0.827 & +0.003 [-0.006, +0.012] & 0.476 & 1.00 & 0.72 \\
MOOC & MC & 0.957 & SASRec & 0.981 & +0.024 [+0.020, +0.028] & $<$0.001 & 0.98 & 0.72 \\
\bottomrule
\end{tabular}

